Out of Sight, Still at Risk: The Lifecycle of Transitive Vulnerabilities in Maven

The modern software development landscape heavily relies on transitive dependencies. They enable seamless integration of third-party libraries. However, they also introduce security challenges. Transitive vulnerabilities that arise from indirect dependencies expose projects to risks associated with Common Vulnerabilities and Exposures (CVEs). It happens even when direct dependencies remain secure. This paper examines the lifecycle of transitive vulnerabilities in the Maven ecosystem. We employ survival analysis to measure the time projects remain exposed after a CVE is introduced. Using a large dataset of Maven projects, we identify factors that influence the resolution of these vulnerabilities. Our findings offer practical advice on improving dependency management.

==> 2-methods_model_gamma.tex <==
\section{Proposed Model}
\label{subsec:ProposedModel}

We propose a mathematical model to explain the observed phenomenon in the data.
The dependency between revisions is represented as a directed acyclic graph $G = (V, E)$, where each node $v \in V$ represents a software component or package, and each edge $(u \to v) \in E$ indicates that $v$ depends on $u$.
Each node $v$ releases new versions at certain time intervals, modeled as stochastic processes or deterministic schedules.
When a vulnerability is discovered and fixed in a base component $v_0$, the fix must propagate to all dependent components that use $v_0$ directly or indirectly.

\paragraph{Explanation: Memoryless Property}
\textbf{The memoryless property} signifies that future events are independent of past events, given the current state.
Formally, for the exponential distribution, this property is expressed as:
$$
P(T > s + t \mid T > s) = P(T > t)
$$
where $T$ is a random variable representing the waiting time.
This property implies that the probability of an event occurring in the next interval $t$ is independent of how much time has already elapsed.

\paragraph{Exponential Distribution ($\alpha = 1$)}
The exponential distribution is a special case of the Gamma distribution that uniquely possesses the memoryless property.
Specifically, when the shape parameter $\alpha = 1$, the Gamma distribution simplifies to the exponential distribution:
$$
T \sim \text{Gamma}(1, \beta) \equiv T \sim \text{Exponential}(\beta)
$$
In this scenario, the Gamma distribution maintains the memoryless property, aligning with the intuition for single-stage processes, such as a single stage of vulnerability resolution.
This makes the exponential distribution ideal for modeling scenarios where the process involves only one independent step.


\paragraph{Gamma Distribution ($\alpha > 1$)}
For $\alpha > 1$, the Gamma distribution models the sum of $\alpha$ independent exponential random variables, which corresponds to multi-stage vulnerability resolution processes.
In such cases, the Gamma distribution \textbf{does not possess} the memoryless property.
This implies that future events, specifically the time to resolve a vulnerability, are dependent on past events, thereby reflecting more complex, multi-stage resolution processes.

In the context of vulnerability resolution modeling in software dependencies, utilizing the Gamma distribution with $\alpha > 1$ mirrors the reality that resolving vulnerabilities typically requires multiple stages—such as identification, patch development, testing, and deployment.
Each of these stages can be modeled as separate steps with their own waiting times.
Consequently, since the resolution process is multi-stage, the total time to resolve a vulnerability depends on the time spent on preceding stages.
This dependency is realistic because delays or inefficiencies in one stage can directly impact the overall resolution time.


\subsection{Justification for Using the Gamma Distribution}
\label{subsec:GammaJustification}

In econometrics and reliability engineering, the Gamma distribution is frequently employed to model waiting times until an event occurs, such as the time until death or failure of a component.
Similarly, in the context of software engineering, the Gamma distribution aptly models the \textbf{resolution time}---the duration required to address and fix a discovered vulnerability within a software component or its dependencies.
Below, we elucidate both the intuitive and mathematical reasons for adopting the Gamma distribution in our model.


\subsubsection{Intuitive Rationale}

The Gamma distribution offers significant flexibility in shape due to its two parameters—the shape parameter ($\alpha$) and the rate parameter ($\beta$).
This flexibility allows it to model a wide range of distribution shapes, accommodating various real-world scenarios.
For instance, software vulnerability resolution times often exhibit right skewness, where most vulnerabilities are resolved relatively quickly, but a few take significantly longer due to complexities in dependencies.
The Gamma distribution naturally captures this skewness, making it well-suited for such data.
Additionally, by tuning the shape parameter, the Gamma distribution can represent different levels of variability in resolution times, reflecting the diverse nature of software components and their dependencies.

Resolving a vulnerability in a software component typically involves multiple sequential steps, such as identifying the vulnerability, developing a fix, testing the fix, and deploying the update.
The Gamma distribution is particularly suitable for modeling the total time of such multi-stage processes.
Each stage can be considered an independent step contributing to the overall resolution time, and the Gamma distribution effectively aggregates these contributions into a single, coherent model.

Moreover, resolution times are inherently positive, and the Gamma distribution is defined only for positive real numbers, ensuring that the model aligns with the nature of the data.
This property eliminates the possibility of negative waiting times, which are not meaningful in this context.

Finally, the parameters of the Gamma distribution provide meaningful interpretations in the context of vulnerability resolution.
The shape parameter ($\alpha$) represents the number of stages or processes involved in resolving a vulnerability, while the rate parameter ($\beta$) is inversely related to the speed of resolution.
This relationship allows us to model how dependency depth affects resolution times, with deeper dependencies potentially leading to slower resolutions.


\subsubsection{Mathematical Justification}

The Gamma distribution can be mathematically justified in our model through its relationship with exponential random variables.
Specifically, the Gamma distribution can be viewed as the distribution of the sum of $\alpha$ independent and identically distributed exponential random variables, each with rate $\beta$.
This property aligns with the multi-stage nature of vulnerability resolution.
If each step in the resolution process (e.g., identification, fixing, testing) is modeled as an exponential waiting time, the total resolution time, being the sum of these independent steps, follows a Gamma distribution.

Mathematically, if we denote each stage's waiting time as $X_i \sim \text{Exponential}(\beta(u))$ for $i = 1, 2, \dots, \alpha$, then the total resolution time $T_u$ is given by:
$$
T_u = X_1 + X_2 + \dots + X_\alpha
$$
Consequently, the sum of these independent exponential random variables follows a Gamma distribution:
$$
T_u \sim \text{Gamma}(\alpha, \beta(u))
$$
This formulation effectively captures the cumulative effect of multiple stages in the resolution process, where each stage contributes to the overall waiting time in a manner that is both mathematically sound and reflective of real-world processes.

Additionally, the Gamma distribution extends the memoryless property of the exponential distribution by allowing the "memory" to build up over multiple stages.
While the exponential distribution is memoryless, meaning that the probability of an event occurring in the next instant is independent of the past, the Gamma distribution accounts for the dependencies introduced by multiple stages.
This is particularly relevant in software vulnerability resolution, where each subsequent step may depend on the completion of previous steps, thereby introducing a dependency structure that the Gamma distribution can effectively model.

The expected value and variance of the Gamma distribution further support its suitability for our model. The expected resolution time is given by:
$$
\mathbb{E}[T_u] = \frac{\alpha}{\beta(u)}
$$
This linear relationship between the expected resolution time and the shape parameter $\alpha$ supports the notion that more complex vulnerabilities (modeled by higher $\alpha$) take longer to resolve.
The variance is given by
$$
\text{Var}(T_u) = \frac{\alpha}{\beta(u)^2}
$$
The variance increases with both the shape parameter and decreases with the square of the rate parameter, indicating greater uncertainty in resolution times for more complex dependencies.

Furthermore, the parameters $\alpha$ and $\beta(u)$ have clear interpretations within the context of software vulnerability resolution.
The shape parameter ($\alpha$) represents the inherent complexity or number of steps in the resolution process, while the rate parameter ($\beta(u)$) reflects the efficiency of the resolution process for a given dependency depth.
As dependency depth increases, $\beta(u)$ decreases, leading to longer expected resolution times, which aligns with the practical challenges encountered in resolving deeply nested dependencies.

\begin{theorem}
\label{theorem:GammaJustification}
In the context of software vulnerability resolution, if the resolution process can be decomposed into $\alpha$ independent sequential stages, each requiring an exponentially distributed amount of time with rate $\beta(u)$, then the total resolution time $T_u$ follows a Gamma distribution with parameters $\alpha$ and $\beta(u)$.
\end{theorem}

\begin{proof}
Assume the resolution process consists of $\alpha$ independent stages, where the time taken to complete each stage is an independent random variable $X_i$ following an Exponential distribution with rate $\beta(u)$:
$$
X_i \sim \text{Exponential}(\beta(u)), \quad i = 1, 2, \dots, \alpha
$$
The total resolution time $T_u$ is the sum of these independent exponential random variables:
$$
T_u = \sum_{i=1}^\alpha X_i.
$$
The sum of $\alpha$ independent Exponential($\beta(u)$) random variables follows a Gamma distribution with shape parameter $\alpha$ and rate parameter $\beta(u)$:
$$
T_u \sim \text{Gamma}\big(\alpha, \beta(u) \big).
$$
This concludes the proof, establishing that under the assumption of independent sequential stages with exponential waiting times, the total resolution time naturally follows a Gamma distribution.
\end{proof}

This justifies assumption .

The \textbf{resolution rate} $\beta(u)$ for a vulnerability in library $u$ is modeled as an inverse function of its dependency depth
$$
\beta(u) = \frac{k}{d(u) + c},
$$
where $k > 0$ is a constant representing the base resolution rate and $d(u)$ is the dependency depth of $u$.
This ensures that $\beta(u)$ decreases as the dependency depth increases, reflecting the increased complexity in resolving vulnerabilities in more deeply nested dependencies.

Let $T_u$ be the resolution time, i.e., a random variable representing the time until a vulnerability in library $u$ is resolved.
We assume that $T_u$ follows a Gamma distribution with shape parameter $\alpha$ and rate parameter $\beta(u)$, denoted as $T_u \sim \text{Gamma}(\alpha, \beta(u))$.
The probability density function (PDF) of $T_u$ is given by:
$$
f_{T_u}(t) = \frac{\beta(u)^\alpha t^{\alpha - 1} e^{-\beta(u) t}}{\Gamma(\alpha)}, \quad t \geq 0,
$$
where $\Gamma(\alpha)$ is the Gamma function.

\subsection{Theorem: Linear Dependence}
\label{theorem:linear_dependence}

Within the defined graph-based probabilistic model, the \textbf{expected resolution time} $\mathbb{E}[T_u]$ of a vulnerability in library $u$ is \textbf{linearly dependent} on its \textbf{dependency depth} $d(u)$.
Mathematically, this relationship is expressed as
$$
\mathbb{E}[T_u] = \frac{\alpha (d(u) + c)}{k},
$$
where $\alpha > 0$ is the shape parameter of the Gamma distribution and $k > 0$ is the constant from Definition \ref{def:resolution_rate}.

\begin{proof}
Given that $T_u \sim \text{Gamma}(\alpha, \beta(u))$, the expected value of $T_u$ is
$$
\mathbb{E}[T_u] = \frac{\alpha}{\beta(u)}.
$$
Substituting $\beta(u)$ from Definition \ref{def:resolution_rate}, we get
$$
\mathbb{E}[T_u] = \frac{\alpha}{\frac{k}{d(u) + c}} = \frac{\alpha (d(u) + c)}{k} = a d(u) + b,
$$
where $a = \frac{\alpha}{k}$ and $b = \frac{\alpha c}{k}$.
\end{proof}

\begin{remark}
Theorem \ref{theorem:linear_dependence} formalizes the intuitive notion that libraries with deeper dependencies ($d(u)$) require longer times to resolve vulnerabilities.
The linear relationship $\mathbb{E}[T_u] = \frac{\alpha (d(u) + c)}{k}$ quantifies this dependence, indicating that each unit increase in dependency depth results in an increase of $\frac{\alpha}{k}$ units in the expected resolution time.
\end{remark}

By selecting the Gamma distribution to model resolution times, the proposed model leverages its inherent flexibility, mathematical properties, and alignment with real-world multi-stage processes.
This choice enables a nuanced and accurate representation of how dependency depth influences vulnerability resolution, providing both theoretical rigor and practical applicability.
The linear dependence of expected resolution time on dependency depth, as established in Theorem \ref{theorem:linear_dependence}, further underscores the suitability of the Gamma distribution in capturing the dynamics of software dependency hierarchies.



==> model.tex <==

\subsection{Proposed model}%
\label{subsec:Proposed model}

We propose a mathematical model that explains the phenomenon observed in the data.
Let the dependency between revisions is represented as directed acyclic graph $G = (V, E)$ where each node $v \in V$ represents a software component or package, and each edge $(u \to v) \in E$ indicates that $v$ depends on $u$.
Each node $v$ releases new versions at certain time intervals, which we can model as stochastic processes or deterministic schedules.
When a vulnerability is discovered and fixed in a base component $v_0$, the fix must propagate to all dependent components that use $v_0$ directly or indirectly.

\begin{definition}[Resolution Rate]
\label{def:resolution_rate}
The \textbf{resolution rate} $\lambda(u)$ for a vulnerability in library $u$ is modeled as an inverse function of its dependency depth
\[
\lambda(u) = \frac{k}{d(u) + 1},
\]
where $k > 0$ is a constant representing the base resolution rate and $d(u)$ is dependency depth. 
\end{definition} 
This rate captures the increased complexity and resource requirements associated with resolving vulnerabilities in more deeply nested dependencies.


Let $T_u$ be the resolution time, i.e. a random variable representing the time until a vulnerability in library $u$ is resolved.
We assume that the resolution time $T_u$ follows an exponential distribution, implying a memoryless property where the probability of resolving the vulnerability in the next instant is independent of the time already spent.
Therefore, its probability density function (PDF) is given by
$$
f_{T_u}(t) = \lambda(u) e^{-\lambda(u) t}, \quad t \geq 0.
$$


\begin{theorem}[Linear Dependence]
\label{theorem:linear_dependence}
Within the defined graph-based probabilistic model, the \textbf{expected resolution time} $\mathbb{E}[T_u]$ of a vulnerability in library $u$ is \textbf{linearly dependent} on its \textbf{dependency depth} $d(u)$.
Mathematically, this relationship is expressed as:
\[
\mathbb{E}[T_u] = \frac{d(u) + 1}{k},
\]
where $k > 0$ is the constant from Definition \ref{def:resolution_rate}.
\end{theorem}


\begin{proof}
Using the assumptions that random variable $T_u$ is exponentially distributed with resolution rate $\lambda(u)$ given by Definition \ref{def:resolution_rate}, we have
\[
\mathbb{E}[T_u] = \frac{1}{\lambda(u)} = \frac{1}{\frac{k}{d(u) + 1}} = \frac{d(u) + 1}{k}.
\]
\end{proof}

\begin{remark}
Theorem \ref{theorem:linear_dependence} formalizes the intuitive notion that libraries with deeper dependencies (higher $d(u)$) require longer times to resolve vulnerabilities. The linear relationship $\mathbb{E}[T_u] = \frac{d(u) + 1}{k}$ quantifies this dependence, indicating that each unit increase in dependency depth results in an increase of $\frac{1}{k}$ units in the expected resolution time.
\end{remark}

\paragraph{Implications of the Linear Relationship}

The established linear relationship has several practical implications.
Firstly, organizations can allocate resources more effectively by anticipating longer resolution times for vulnerabilities in libraries with higher dependency depths.
Secondly, vulnerabilities in libraries with lower dependency depths can be prioritized for quicker resolution, thereby enhancing overall system security.
Lastly, policies can be formulated to address vulnerabilities systematically based on their dependency depths, ensuring that critical dependencies are managed proactively.

